Revisiting Code Similarity Evaluation with Abstract Syntax Tree Edit Distance

This paper revisits recent code similarity evaluation metrics, particularly focusing on the application of Abstract Syntax Tree (AST) editing distance in diverse programming languages. In particular, we explore the usefulness of these metrics and compare them to traditional sequence similarity metrics. Our experiments showcase the effectiveness of AST editing distance in capturing intricate code structures, revealing a high correlation with established metrics. Furthermore, we explore the strengths and weaknesses of AST editing distance and prompt-based GPT similarity scores in comparison to BLEU score, execution match, and Jaccard Similarity. We propose, optimize, and publish an adaptable metric that demonstrates effectiveness across all tested languages, representing an enhanced version of Tree Similarity of Edit Distance (TSED).

==> latex/approaches_copy.tex <==
% We propose a novel metric that we name Tree Similarity of Editing Distance (TSED)\footnote{https://github.com/Etamin/TSED} to assess the similarity between two SQL queries. This innovative approach, illustrated in Figure \ref{fig:tsed}, encompasses three distinct stages to provide a comprehensive evaluation. The initial stage involves the transformation of the two SQL queries into Abstract Syntax Trees (ASTs), facilitating a structured comparison. Following this, we calculate the editing distance between these ASTs, capturing the extent of their dissimilarity. The final step involves normalizing this distance measure to a scale between 0 and 1, allowing for a straightforward and interpretable assessment of query similarity.
\begin{figure}[htb]
\centering
\includegraphics[width=\columnwidth]{figures/tsed.drawio.pdf}
\caption{Pipeline of TSED Code Evaluation Metric}
\label{fig:tsed}
\end{figure}

\noindent % \paragraph{SQL Parsing and Its Mathematical Interpretation}
\textbf{Code Parsing: A Mathematical Perspective}
Parsing code into an AST is a fundamental process in understanding and analyzing the structure of programming code and it is the first step to get AST editing distance. In this procedure, the code is transformed from its raw textual form into a hierarchical tree-like structure that represents the syntactic structure of the code. This transformation aids in capturing the relationships and dependencies among different elements of the code, facilitating subsequent analysis and manipulation. The mathematical abstraction of this process involves the application of formal grammars, particularly context-free grammars, to define the syntax of the programming language. Parsing algorithms, such as the widely used LL (left-to-right, leftmost derivation) or LR (left-to-right, rightmost derivation) parsing techniques, implement these grammars to generate the AST. The AST is then constructed by recursively applying these parsing rules, resulting in a structured representation that mirrors the hierarchical organization of the code. 

\noindent
% \textbf{Parser Solutions:} One of the contemporary tools addressing this challenge is the \texttt{@florajs/sql-parser}\footnote{https://github.com/florajs/sql-parser}. Beyond traditional parsing, this tool embeds a nuanced transformation function . 
\textbf{Parser Solutions:}
\yw{How tree-sitter works and how the different to SQL parsing}
% If we consider \( \mathcal{S} \) as the space encompassing all code strings, this transformation function creates a bridge from any SQL string \( s \) in \( \mathcal{S} \) to its corresponding AST, \( a \), in \( \mathcal{A} \):

% \begin{equation}
% a = T(s) \quad \text{where} \quad s \in \mathcal{S} \, \text{and} \, a \in \mathcal{A}
% \end{equation}
% We describe its cardinality,  $|\mathcal{A}|$, using an indicator function  $\delta$ to highlight the uniqueness of each AST:

% \begin{equation}
% |\mathcal{A}| = \sum_{i=1}^{n} \delta(A_i) \quad \text{where} \quad \delta(A_i) = 
% \begin{cases} 
% 1, & \text{if } A_i \text{ is unique within } \mathcal{A}\\
% 0, & \text{otherwise}
% \end{cases}
% \end{equation}

% Given the complexity and multifaceted nature of SQL, \textit{n}, which represents the conceivable number of unique AST structures, can be dauntingly large. This observation accentuates the pivotal role of the \texttt{@florajs/sql-parser}, ensuring parsing processes are both rigorous and efficient.

\noindent %\paragraph{Tree Synthesis from Abstract Syntax Trees}

% Summarily, this synthesis process metamorphoses the linear SQL query representations into a hierarchical topological format, serving as the cornerstone for subsequent intricate analytical procedures in the project.


\noindent
\textbf{Tree Distance Computation.}
% One of the fundamental challenges in comparing trees, especially those derived from SQL queries, is quantifying their similarity or difference. Here, the concept of tree edit distance comes into play.

% The tree edit distance between two trees \( T_1 \) and \( T_2 \) measures the minimum number of basic edit operations (insertion, deletion, and renaming of nodes) required to transform \( T_1 \) into \( T_2 \). Mathematically, the tree edit distance function \( \Delta \) can be defined as:
% \vspace{-0.1cm}
% \begin{equation}
% \Delta(T_1, T_2) = \min_{ops} \sum_{i=1}^{n} w(op_i)
% \end{equation}
% where  \textit{ops} is a sequence of \textit{n} edit operations that transform  $T_1$ to $T_2$, and $w(op_i)$ is the cost associated with the  $i^{th}$ operation. The goal is to find the sequence of operations that minimizes the total cost.

% However, computing the tree editing distance is computationally intensive. The problem is NP-hard, and naive algorithms have a time complexity that is doubly exponential in the size of the trees. Let $|T_1|$ and $|T_2|$ denote the sizes of trees $T_1$ and $T_2$ respectively. The computational complexity $\mathcal{C}$ can be represented as:

% \begin{equation}
% \mathcal{C}(|T_1|, |T_2|) = \mathcal{O}\left(2^{2^{|T_1| + |T_2|}}\right)
% \end{equation}

% Given the need for efficient computation, we employ the `APTED' algorithm~\cite{pawlik2016tree}~\cite{pawlik2015efficient}, a state-of-the-art tool designed for tree edit distance computation. The library optimizes the process using advanced algorithms and data structures, significantly reducing computational time. In our project, the `APTED' function compute the distance, the return $\delta$ will be an integer:
% $\delta = APTED(T_1, T_2)$, where  $\delta$ represents the tree edit distance between $T_1$ and $T_2$.

% In essence, tree edit distance provides a robust metric to quantify the similarity between SQL query structures, and the `apted' library facilitates its efficient computation, enabling a deeper understanding and comparison of different SQL queries.
Quantifying the similarity or difference between trees, particularly those derived from SQL queries, is a fundamental challenge, and the concept of tree edit distance addresses this issue. The tree edit distance $\Delta(T_1, T_2)$ between two trees $T_1$ and $T_2$ measures the minimum number of basic edit operations (insertion, deletion, and renaming of nodes) required for the transformation. Mathematically, it can be defined as:
\vspace{-0.1cm}
\begin{equation}
\Delta(T_1, T_2) = \min_{ops} \sum_{i=1}^{n} w(op_i)
\end{equation}
where $ops$ is a sequence of $n$ edit operations, and $w(op_i)$ is the cost associated with the $i^th$ operation.
To address this, we employ the same APTED algorithm~\cite{pawlik2016tree}~\cite{pawlik2015efficient}, a state-of-the-art tool for efficient tree edit distance computation to original TSED work. Represented as $\delta = APTED(T_1, T_2)$, where  $\delta$ represents the tree edit distance between $T_1$ and $T_2$.
\textbf{Normalization.}

Beyond merely calculating the raw editing distance, we take into account the complexity of the queries by normalizing the distance using the maximum number of tree nodes and we add a different situation than original:  
\begin{equation}
\begin{aligned}
\beta=MaxNodes(T_1, T_2) \\
TSED = 
\begin{cases} 
\delta/\beta , & \text{if } \beta  > \delta \\
0, & \text{otherwise}
\end{cases}
\end{aligned}
\end{equation}
This normalization allows us to obtain a more comprehensive and meaningful final result, as it accounts for variations in query complexity and structure. 
% By computing the distance-to-maximum-nodes ratio, we arrive at a final evaluation metric that offers a nuanced perspective on the accuracy and efficiency of our Text2SQL conversion techniques. This approach ensures that our assessments are not only sensitive to the accuracy of the conversions but also consider the relative complexity of queries, enabling a more balanced and informative measure of performance.
